Attribute Inference Attacks for Federated Regression Tasks

Federated Learning (FL) enables multiple clients, such as mobile phones and IoT devices, to collaboratively train a global machine learning model while keeping their data localized. However, recent studies have revealed that the training phase of FL is vulnerable to reconstruction attacks, such as attribute inference attacks (AIA), where adversaries exploit exchanged messages and auxiliary public information to uncover sensitive attributes of targeted clients. While these attacks have been extensively studied in the context of classification tasks, their impact on regression tasks remains largely unexplored. In this paper, we address this gap by proposing novel model-based AIAs specifically designed for regression tasks in FL environments. Our approach considers scenarios where adversaries can either eavesdrop on exchanged messages or directly interfere with the training process. We benchmark our proposed attacks against state-of-the-art methods using real-world datasets. The results demonstrate a significant increase in reconstruction accuracy, particularly in heterogeneous client datasets, a common scenario in FL. The efficacy of our model-based AIAs makes them better candidates for empirically quantifying privacy leakage for federated regression tasks.

==> sources/acknowledgements.tex <==
\section{Acknowledgements}\label{sec:acks}
This research was supported in part by the Groupe La Poste, sponsor of the Inria Foundation, in the framework of the FedMalin Inria Challenge, as well as by the France 2030 program, managed by the French National Research Agency under grant agreements No. ANR-21-PRRD-0005-01, ANR-23-PECL-0003, and ANR-22-PEFT-0002. It was also funded in part by the European Network of Excellence dAIEDGE under Grant Agreement Nr. 101120726, by SmartNet and LearnNet, and by the French government National Research Agency (ANR) through the UCA JEDI (ANR-15-IDEX-0001), EUR DS4H (ANR-17-EURE-0004), and the 3IA Côte d’Azur Investments in the Future project with the reference number ANR-19-P3IA-0002. \\
The authors are grateful to the OPAL infrastructure from Université Côte d'Azur for providing resources and support.

==> sources/attacks.tex <==


\section{Model-based AIA guarantees for  least squares regression.}
\label{sec:model-based-guarantees}
In this section, 
%we will demonstrate the motivation of utilizing model-based AIA for federated regression problems. 
%First, we illustrate that the performance of gradient-based AIA~\cite{attribute_fl} is not always correlated with gradient's similarity for regression. 
we provide novel theoretical guarantees for the accuracy of the model-based AIA (Problem~\eqref{eq:aia_model_based}) in the context of least squares regression.  In particular, we show that the better the model $\model$ fits the local data and the more the sensitive attribute affects the final prediction, the higher the AIA accuracy.
 


%\subsection{Model-based AIA guarantees for least squares regression.}
\begin{prop}\label{prop:attribute_nonprivate}
%Let $\s $ be the vector including all the unknown sensitive binary attributes $\{s_c(i), \forall i\in \{1, ..., S_c\}\}$ of client $c$.
Let $E_c$ be the mean square error of a given least squares regression model $\model$ on the local dataset of client $c$ and $\model[s]$ be the model parameter corresponding to a binary sensitive attribute. The accuracy of the model-based AIA \eqref{eq:aia_model_based} is larger than or equal to $1-\frac{4E_c}{\model[s]^2}$. 
\end{prop}

\begin{proof}
Let $\s $ be the vector including all the unknown sensitive binary attributes $\{s_c(i), \forall i\in \{1, ..., S_c\}\}$ of client $c$.
Let $\x\in \real^{S_c\times d}$ be the design matrix with rank $d$ and $\y\in \real^{S_c}$ be the labels in the local dataset $\localdataset$ of the client $c$.  Let $\model[:p]\in \real^{d-1}$ be the parameters corresponding to the public attributes. 
The adversary has access to partial data instances in $\localdataset$ which consists of the public attributes $\P\in \real^{S_c\times(d-1)}$ and the corresponding labels $\y\in \real^{S_c}$. 

The goal for the adversary is to decode the values of the binary sensitive attribute $\s \in\{0,1\}^{S_c}$ given $(\P, \y)$ by solving~\eqref{eq:aia_model_based}, i.e., checking for each point, which value for the sensitive attribute leads to a smaller loss.

It is easy to check that the problem can be equivalently solved through the following two-step procedure.
First, the adversary computes the vector of real values:
$$
\tilde{\mathbf{s}}_c = \argmin_{\s\in \real^{S_c}} ||\P\model[:p]+ \s\model[s] - \y ||_2^2 = \frac{\y-\P\model[:p]}{\model[s]}.  
$$
Then, the adversary reconstruct the vector of sensitive features $\hat{\mathbf{s}}_c \in \{0,1\}^{S_c}$ as follows
\begin{equation}\label{eq:sensitive_prediction_condition}
\hat s_c(i) = 
\begin{cases}
    0& \text{if } \tilde{{s}}_c(i) <\frac{1}{2}\\
    1              & \text{otherwise}
\end{cases}
,\,\,\,\forall i\in \{1, ..., S_c\}. 
\end{equation}


% Note that this approach yields the same solution as picking the sensitive attribute, which leads to the smaller loss. 

%Now we start to evaluate the difference between the recovered $\hat{\mathbf{s}}_c$ and the true labels $\s$.
Let $\e$ be the vector of residuals for the local dataset, i.e., $\e_c = \y - (\P\model[:p]+ \s\model[s])$. We have then 
\begin{equation}\label{eq:sensitive_relation}
    \s = \frac{\y - \P \model[:p] - \e_c}{\model[s]} = \tilde{\mathbf{s}}_c - \frac{\e_c}{\model[s]}. 
\end{equation}

Let us say that the sensitive feature of sample $i$ has been erroneously reconstructed, i.e., $s_c(i) \neq \hat s_c(i)$, then  \eqref{eq:sensitive_prediction_condition}, implies that $|s_c(i) - \tilde s_c(i)|\ge 1/2$, and from
 \eqref{eq:sensitive_relation} it follows that $|e_c(i)|^2 \ge \model[s]^2/4$. As $E_c S_c= \lVert \e_c \rVert_2^2$, there can be at most $4 E_c S_c/\model[s]^2$ samples erroneously reconstructed, from which we can conclude the result.
 \end{proof}

% According to Eqs.~\ref{eq:sensitive_prediction_condition} and~\ref{eq:sensitive_relation}, we know that the prediction entry in $\hat{\mathbf{s}}_c$ differs from $\s$ only when the corresponding entry in $\frac{\e}{\model[s]}$ has an absolute value above $1/2$. Let $E_c$ be the mean square error of the accessible data instance, i.e.,~$E_c = \frac{||\e||_2^2}{S_c}$.
% We have $||\e||_2^2 = E_c \times S_c$ and $||\frac{\e}{\model[s]}||_2^2 =  \frac{E_c \times  S_c}{\model[s]^2}$. This implies that $\frac{\e}{\model[s]}$ cannot have more than
% $\lfloor\frac{4E_c \times S_c}{\model[s]^2}\rfloor$ entries with absolute value above $1/2$. Therefore, the success of the attack is larger than or equal to $1-\frac{4E_c}{\model[s]^2}$.


%From Proposition~\ref{prop:attribute_nonprivate}, we can see that the accuracy of the attack depends on the importance of the sensitive attribute in model $\model$ and how well the model fits the data. If the model fits perfectly the known data, the attack can achieve $100\%$ of the accuracy on these data.
%This result suggests that AIA on models do not suffer the limit of AIA on gradients, namely their sensitivity to the dataset size. 

Proposition~\ref{prop:attribute_nonprivate} indicates that the model-based AIA performs better the more the model overfits the dataset.
This observation justifies the following two-step attack in a FL setting: 
\emph{the adversary first reconstructs the optimal local model of the targeted client $c$, i.e., $\localmodel = \arg\min_{\model\in \real^d} \locallossfunction(\model, \localdataset)$, and then execute the AIA in \eqref{eq:aia_model_based} on the  reconstructed model.}\footnote{
Note that this model is optimal in terms of the training error, but not in general of the final test error. On the contrary, it is likely to overfit the local dataset.
}
In the following, we will detail our approaches for reconstructing the optimal local model by passive and active adversary, respectively.    
%We refer to the first step as the \emph{local model reconstruction attack} (LMRA).

% the more the model overfits the local 
% Our theoretical finding motivates the adversary in FL to trigger AIA on a model with a small loss error, i.e., on a model overfitting the client's dataset. Therefore, in the context of FL, to enhance the model-based AIA performance, the adversary should first reconstruct the optimal local model of the targeted client, $c$, i.e., $\localmodel = \arg\min_{\model\in \real^d} \locallossfunction(\model, \localdataset)$, and then execute the model-based AIA using the reconstructed model. We name this attack the local model reconstruction attack.

%During the federated training process, the adversary can directly execute this model-based AIAs on the global model  $\model^T$ or the last-returned model $\model_c^T(K)$. We can see from Figure~\ref{fig:gradient_vs_model} that the model-based AIAs outperform the gradient-based AIA, once the local dataset size is twice larger than the batch size. The performance of gradient-based AIA is more significantly influenced by the dataset size, which drops from $70\%$ to around $50\%$ when the dataset size increases from 32 to 256. 






\section{Reconstructing the local model  in FL}\label{sec:lmra}
In this section, we show how an adversary may reconstruct the optimal local model of client $c$, i.e.,~$\localmodel = \arg\min_{\model\in \real^d} \locallossfunction(\model, \localdataset)$.

First, we provide an efficient approach for least squares regression under a passive adversary. We prove that the adversary can exactly reconstruct the optimal local model under deterministic FL updates and provide probabilistic guarantees on the reconstruction error under stochastic FL updates (Sec.~\ref{sec:exact}).

Second, we show that an active adversary can potentially reconstruct any client's local model (not just least square regression ones) in a federated setting 
% , for general ML models, the this attack can be more easily carried out by a malicious adversary, and we provide a solution to make the attack less detectable for any machine learning model trained in a federated manner 
(Sec.~\ref{subsec:active}).


\subsection{Passive approach for linear least squares}\label{sec:exact}

We consider that clients cooperatively train a linear regression model with quadratic loss. We refer to this setting as a federated least squares regression.  % $\localdataset$.
The attack is detailed in Alg.~\ref{algo:lineardecode} and  involves a single matrix computation (line~\ref{algoline:ols}) after the exchanged messages $\messages_c$ have been collected. $\mathbf{A}^\dagger$ represents the pseudo-inverse of matrix $\mathbf{A}$.  
Theorem~\ref{prop:stochastic_case} provides theoretical guarantees  for the distance between the reconstructed model and the optimal local one, when the model is trained through FedAvg~\cite{mcmahan2017communication} with batch size $B$ and local epochs $E$. The formal statement of the theorem and its proof are in Appendix~\ref{app:stochasticproof}.

\begin{algorithm}[t]
\caption{Reconstruction of client-$c$ local model by a passive adversary for federated least squares regression }\label{algo:lineardecode}
\textbf{Input}: 
    the server models $\model^{t_i}(0)=\model_c^{t_i}(0)$ and the local updated models  $\model_c^{t_i}(K)$ at all the inspected rounds $t_i\in  \mathcal{T}_c= \{t_1, t_2, \dots, t_{n_c}\} $.
\begin{algorithmic}[1]
\small
    \STATE{Let $\Theta_{\text{in}}=[\model_c^{t_1}(0) \,\, \model_c^{t_2}(0) \,\, ... \,\, \model_c^{t_{n_c}}(0)]^T \in \real^{n_c\times{d}}$}
    \STATE{Let ${\Theta_{\text{out}}= \left[\begin{array}{cc}(\model_c^{t_1}(0)-\model_c^{t_1}(K))^{T} & 1 \\ \vdots & \\ (\model_c^{t_{n_c}}(0)-\model_c^{t_{n_c}}(K))^{T} & 1\end{array}\right] \in \real^{n_c\times(d+1)}}$}
    \STATE{
        ${(\hat\model_c^*)^T \leftarrow \text{last row of} \left( (\Theta_{\text{out}}^T \Theta_{\text{out}})^{\dagger}\Theta^T_{\text{out}}\Theta_{\text{in}} \right)}$ %\in \real^{(d+1)\times d}}$ 

    }\label{algoline:ols}
    
    \STATE{Return $\hat \model_c^*$ as the estimator for client $c$'s local model}
    
\end{algorithmic}
\end{algorithm}


%If the attacked client's  updates are random, e.g., due to batch sampling, the adversary can still  reconstruct the client's optimal local model with high probability.

% THEOREM BEFORE FRANCESCO'S MODIFICATIONS
% \begin{theorem}[Informal statement]\label{prop:stochastic_case}    
% Consider a federated least squares regression with a large number of clients and assume that i)~client $c$ has $d$-rank design matrix $\x \in \real^{S_c\times d}$, ii)~she updates the global model through stochastic gradient steps  with sub-Gaussian noise with scale $\sigma$ and small learning rate $\eta$, and iii)~the local data distribution of the targeted client is different from the global data distribution. By eavesdropping on $n_c>d$ message exchanges between client $c$ and the server, 
% the error of the reconstructed model $\hat\model^*_c$ of Algorithm~\ref{algo:lineardecode} is upper bounded w.p.  $\ge 1-\delta$  when $\eta\leq \frac{S_c}{2\lambda_{\max}(\x^T\x)}$ and
% \begin{equation}\label{eq:bounds}
%   \left\lVert \hat\model^*_c - \localmodel \right\rVert_2 = \mathcal{O}\left(\eta\sigma d\sqrt{  dE\left\lceil\frac{S_c}{B}\right\rceil \frac{d+1+\ln \frac{2d}{\delta}}{n_c \cdot \underline{\lambda}}} \right). 
% \end{equation}
% \end{theorem}

\begin{theorem}[Informal statement]\label{prop:stochastic_case}    
Consider a federated least squares regression with a large number of clients and assume that i)~client $c$ has $d$-rank design matrix $\x \in \real^{S_c\times d}$, ii)~she updates the global model through stochastic gradient steps  with sub-Gaussian noise with scale $\sigma$ and small learning rate $\eta$, iii)~the global model is independent of previous target client updates, and iv)~the eigenvalues of the matrix $\frac{\Theta_{\text{out}}^{T} \Theta_{\text{out}}}{n_c}$ are lower bounded by $\underline{\lambda}>0$. By eavesdropping on $n_c>d$ message exchanges between client $c$ and the server, the error of the reconstructed model $\hat\model^*_c$ of Alg.~\ref{algo:lineardecode} is upper bounded w.p.  $\ge 1-\delta$  when $\eta\leq \frac{S_c}{2\lambda_{\max}(\x^T\x)}$ and
\begin{equation}\label{eq:bounds}
  \left\lVert \hat\model^*_c - \localmodel \right\rVert_2 = \mathcal{O}\left(\eta\sigma d\sqrt{  dE\left\lceil\frac{S_c}{B}\right\rceil \frac{d+1+\ln \frac{2d}{\delta}}{n_c \cdot \underline{\lambda}}} \right). 
\end{equation}
\end{theorem}


When the batch size is equal to the local dataset size, Alg.~\ref{algo:lineardecode} exactly reconstructs the optimal local model (proof in Appendix~\ref{app:proof_corollary}):
% an exact reconstruction (Proposition~\ref{cor:linear_reconstruction}) which is order-optimal in terms of the number of messages considered (Prop.~\ref{prop:order-optimal}). 

\begin{prop}\label{cor:linear_reconstruction}
Consider a federated least squares regression and assume that client $c$ has $d$-rank design matrix and updates the global model through full-batch gradient updates (i.e., $B=S_c$) and an arbitrary number of local epochs. Once the adversary eavesdrops on $d+1$ communication exchanges between client $c$ and the server, it can recover the client's optimal local model.
\end{prop}

% The formal statement of Theorem~\ref{prop:stochastic_case} and its proof are in Appendix~\ref{app:stochasticproof}. The proof of Proposition~\ref{cor:linear_reconstruction} are in Appendix~\ref{app:proof_corollary}.



Finally, the following proposition shows that 
our attack for the full-batch gradient case is \textbf{order-optimal} in terms of the number of messages the adversary needs to eavesdrop. The proof is in Appendix~\ref{app:proof_proposition}.

\begin{prop}\label{prop:order-optimal}
%For a least squares regression task, let $d$ be the number of the features. 
Consider that the federated least squares regression is trained through FedAvg with one local step ($E=1$) and full batch ($B=S_c$ for each client $c \in \mathcal{C}$).
%For any FL algorithm 
%where a client's local update rule can be seen as a first-order black box,\footnote{For every client $c$, its local model $\model_c(t)$ can be expressed as 
%\begin{equation*}
%    \model_c(t) = \model_c(0) + \textbf{span}\{\nabla\locallossfunction(\model_c(0)),
%\nabla\locallossfunction(\model_c(1)), ...,
%\nabla\locallossfunction(\model_c(t-1))\}.
%\end{equation*}} 
At least one client is required to communicate with the server $\Omega(d)$ times for the global model to be learned, and the adversary needs to eavesdrop at least $\Omega(d)$ messages from this client to reconstruct her optimal local model.
\end{prop}


\paragraph{Toy example illustration} 
Here, we illustrate the performance of our Alg.~\ref{algo:lineardecode} on a toy dataset detailed in Appendix~\ref{app:toydataset}. Figure~\ref{fig:linear_toy} (left) demonstrates that 
as the batch size increases, the reconstructed model is closer to the optimal local model (as shown in our Theorem~\ref{prop:stochastic_case}). Moreover, since the model overfits more the dataset (with smaller loss), the AIA accuracy increases (Figure~\ref{fig:linear_toy} (right)). 
\begin{figure}[htbp]
\begin{subfigure}[t]{0.45\columnwidth}
    \centering
    \includegraphics[scale=0.21]{figures/toy/Passive_linear_LMRA_1.png}
\end{subfigure}
%\hfill
\begin{subfigure}[t]{0.45\columnwidth}
    \centering
    \includegraphics[scale=0.205]{figures/toy/Passive_linear_AIA_1.png}
\end{subfigure}
\caption{The performance of our passive approach for reconstructing optimal local model (left) and the triggered AIA (right) on a toy dataset with two clients training a linear model with size $d=11$ under batch size 64, 256 and 1024 for 5 seeds each, respectively. The passive adversary only eavesdropped $d+1$ messages.}
\label{fig:linear_toy}
\end{figure}


\subsection{Active approach} \label{subsec:active}
Here we consider an active adversary (e.g., the server itself) that can modify the global model weights $\model^t$ to recover the client's optimal local model. 
To achieve this, the adversary can simply send back to the targeted client $c$ her own model $\model_c^{(t-1)}$ instead of the averaged model $\model^t$. In this way, client $c$ is led to compute her own optimal local model.

We propose a slightly more sophisticated version of this active attack. Specifically, we suggest that the adversary emulates the Adam optimization algorithm~\cite{adam} for the model updated by client $c$ by adjusting the learning rate for each parameter based on the magnitude and history of the gradients, and incorporating momentum. The motivation is twofold. First, the client does not receive back exactly the same model and thus cannot easily detect the attack. Second, Adam is known to minimize the training error faster than stochastic gradient descent at the cost of overfitting more to the training data~\cite{adam_generalize_1, adam_generalize}. We can then expect Adam to help the adversary reconstruct the client's optimal local model better for a given number of modified messages, and our experiments in Sec.~\ref{sec:exp}
 confirm that this is the case.

The details of this attack are outlined in Alg.~\ref{algo:active}. We observe that the adversary does not need to systematically modify all messages sent to the target client $c$ but can modify just a handful of messages that are not necessarily consecutive. This contributes to the difficulty of detecting the attack.

% Intuitively, the adversary might attempt to transmit the model derived from the targeted client $c$ (i.e., $\model_c(t-1)$) back to the same client, rather than using the averaged model. However, this strategy can be easily detected by the targeted client.

% In order to address this issue, we propose that the adversary emulates the Adam optimization algorithm~\cite{adam} for the model updated by client $c$, by adjusting the learning rate for each parameter based on the magnitude and history of the gradients and incorporating momentum. 
% The other reasons to choose Adam are that it typically converges faster in practice (i.e., the adversary requires fewer communication rounds for the attack) and that it generalizes poorly compared to the stochastic gradient descent~\cite{adam_generalize_1, adam_generalize} (i.e., the adversary can obtain a model overfitting more the local dataset). 
% We observe that the attacker does not need to modify the messages over consecutive rounds, which makes 

% our attack does not require the adversary to execute the attack in consecutive rounds. Let $\mathcal{T}^a_c$ denote the set of rounds during which the adversary attacks client $c$ and then modify the messages .  While, during the remaining rounds, the adversary operates as a standard server in Algorithm~\ref{algo:fl}.   
% The details of this attack are outlined in Alg.~\ref{algo:active}. 

\begin{algorithm}[t]
\caption{Reconstruction of client-$c$ local model by an active adversary $a$}\label{algo:active}
 \textbf{Input}: Let $\mathcal{T}^a_c $ be set of rounds during which the adversary attacks client $c$ and $\model^a_c$ be the corresponding malicious model.
\begin{algorithmic}[1]
    \STATE{$\model_c^a \leftarrow$ latest model received from client $c$}
    \FOR{$t\in  \mathcal{T}^a_c$}
        \STATE{$a$ sends the model $\model^a_c$ to client $c$,}
        \STATE{$a$ waits the updated model from $\model_c$ %returned 
        from client $c$,}
        \STATE{$a$ computes the pseudo-gradient $\model^a_c-\model_c$ and updates $\model^a_c$ and the corresponding moment vectors following Adam~\cite[Alg.~1]{adam},}
       
    \ENDFOR
\STATE{Return $\model^a_c$ as the estimator for client $c$'s local model}
\end{algorithmic}
\end{algorithm}





% \subsection{General model case}\label{sec:heuristic}
% %In this section, we propose a heuristic (Algorithm~\ref{algo:decode}) for a local model reconstruction attack suited
% %in a more general case , which targets for any FL algorithm falling into the framework in Algorithm~\ref{algo:fl} and any machine learning problem.  

% In this section, we present a heuristic for local model reconstruction attacks (Algorithm~\ref{algo:decode}) applicable to any machine learning models trained using a Federated Learning algorithm that conforms to the framework described in Algorithm~\ref{algo:fl}.


% \begin{algorithm}[t]
% \caption{Local model reconstruction attack}\label{algo:decode}
%     \textbf{Input}: $\message_c=\{(\model (t), \model_c(t)), \forall t\in \roundsclient\}$, the messages inspected by the adversary.\\
%     %\makebox[0pt][l]{}\phantom{Input:       }
% \begin{algorithmic}[1]
%     \STATE{$\Delta \message_c =  \{(\model, \Delta\model = \model_c-\model), \forall (\model, \model_c) \in \message_c\}$}
%     \STATE{Define a mapping function $\mimicfunction_c:\real^m \times \real^d \rightarrow \real^d$ with parameters $\weights\in \real^m$, taking the server model $\model\in \real^d$ as input and predicting the local update, i.e.,~the difference between the local model and the server model.}\label{algoline:gradient_network_def}
%     \STATE{Estimate $\mimicfunction_c$ parameters, by minimizing the empirical risk:
%     \begin{equation}\label{eq:map}
%         \hat w = \arg \min_{w\in \real^m} \sum_{(\model, \Delta \model)\in \Delta \message_c} \left\lVert \mimicfunction_c(w, \model) - \Delta \model \right\rVert ^2   
%     \end{equation}
%     }
%     \STATE{Estimate the model $\hat \model_c$, by minimizing the norm of the local update $\mimicfunction_c$ for fixed parameters $\hat{w}$:
%     %, denoted by 
%     %$\hat \model$, that generates the smallest local update difference:
%     \begin{equation}\label{eq:decode_local_model}
%           \hat \model_c =   \min_{\model \in \real^d} \left\lVert \mimicfunction_c(\hat w, \model) \right\rVert^2
%     \end{equation}
%     }
%     \STATE{Return $\hat \model_c$ as the estimator for the local model of client $c$}
% \end{algorithmic}
% \end{algorithm}
% Our approach for approximately reconstructing the local model of client $c$ consists of two steps. First, the adversary learns a mapping function $\mimicfunction_c(\hat w, \cdot)$ to mimic the local update rule of the client by examining the messages in $\message_c$ (see \eqref{eq:map} in Algorithm~\ref{algo:decode}). Specifically, given the server model $\model$ as input, $\mimicfunction_c(\hat w, \model)$ predicts the client's update $\Delta \model = \model_c - \model$. Second, the adversary estimates the local model of client $c$ as the one that minimizes $\left\lVert \mimicfunction_c(\hat w, \theta) \right\rVert^2$ (see \eqref{eq:decode_local_model} in Algorithm~\ref{algo:decode}). The intuition behind this step is that the client would not update the server model ($\Delta \theta=0$) if it coincides with its optimal local model.


% In general, the performance of our heuristic relies on two factors: 1) the effectiveness of the mapping function $\mimicfunction_c$ in mimicking the specific client's update rule (Algorithm~\ref{algo:fl}, line~\ref{algoline:updaterule}), and 2) the proximity of the estimated $\hat{\model}$ to the true minimizer of Problem~\eqref{eq:decode_local_model} when $||\mimicfunction_c||^2$ is non-convex.

% The first factor depends on the complexity of the learning task, the complexity of the mapping function, the randomness introduced by the client's update rule, and the number of messages observed by the adversary. 
% In particular, the more randomness introduced, the less accurate the estimation of $\mimicfunction_c$, and consequently, the reconstructed local model. Privacy defenses that amplify the randomness in the original algorithm, such as adding noise~\cite{DP}, sub-sampling~\cite{balle2018privacy, wang2019subsampled}, or randomly combining data samples~\cite{mixup, FEDMIX}, are expected to affect the performance of our local model reconstruction attack. 
% In presence of noisy updates, the more messages the adversary can inspect, the closer $\mimicfunction_c$ will resemble the local update rule, resulting in a smaller model reconstruction error (as shown in Proposition~\ref{prop:stochastic_case} for the federated least squares regression). At the same time,  our experimental results suggest that an adversary can reconstruct a neural network model by eavesdropping on merely 10\% of the messages exchanged between the client and the server throughout the entire training process. This number of messages is notably smaller than what one might expect based on the theoretical results (Propositions~\ref{obs:linear_reconstruction} and~\ref{prop:stochastic_case}). Note that one-shot FL algorithms 
% may seem to contrast our attack,  but they might release directly the optimal local model~\cite{zhangdense, fusion}. 

% %The second factor depends on the structure of $\mimicfunction_c$. Our experiments show that our heuristic performs well even when $\mimicfunction_c$ is implemented using a neural network, leading to a highly non-convex Problem~\eqref{eq:decode_local_model}.
% The second factor is influenced by the structure of $\mimicfunction_c$. Experiments in the next section demonstrate that our heuristic exhibits strong performance even when $\mimicfunction_c$ is implemented as a neural network, which results in a highly non-convex Problem~\eqref{eq:decode_local_model}.
% %, and then on the structure of $\mimicfunction_c$.  

 








==> sources/background.tex <==
\section{Preliminaries}\label{sec:prelimi}
\subsection{Federated learning}
We denote by $\clients$ the set of all clients participating to FL. 
Let $\localdataset = \{(\x(i), y_c(i)), i=1,..., S_c\}$ denote the local dataset of client $c\in \clients$ with size $S_c\triangleq |\localdataset|$.  Each data sample $(\x(i), y_c(i))$ is a pair consisting of an input $\x(i)$ and of an associated target value $y_c(i)$.
In FL, clients cooperate to learn a global model, which minimizes the following empirical risk over all the data owned by clients:
\begin{align}
\label{eq:globalobjective}
\min_{\model \in \real^d} \globallossfunction(\model) 
&= \sum_{c \in \clients} p_c \locallossfunction(\model, \dataset_c) \notag \\
&= \sum_{c \in \clients} p_c \left( \frac{1}{S_c} \sum_{i=1}^{S_c} \ell(\model, \x(i), y_c(i)) \right).
\end{align}
%G: THE SECOND FUNCTION ABOVE WAS \locallossfunction, BUT WE DO NOT NEED REALLY THE DEPENDENCE ON C AS WE MAKE EXPLICIT THE SET. I THINK THIS IS A BETTER CHOICE WHEN WE THEN HAVE EQUATIONS LIKE (2) WHERE WHAT MATTERS IS REALLY THE DATASET ON WHICH THE LOSS IS COMPUTED
where $\ell(\model, \x(i), y_c(i))$ measures the loss of the model $\model$ on the sample $(\x(i), y_c(i))\in \localdataset$ and $p_c$ is the positive weight of client $c$, s.t.,~$\sum_{c\in \clients} p_c = 1$. Common choices of weights are $p_c =\frac{1}{|\clients|}$ or $p_c =\frac{S_c}{\sum_{c\in \clients}S_c}$.

\begin{algorithm}[t]
\caption{FL Framework}\label{algo:fl}
\textbf{Output}: $\model^T$
\begin{algorithmic}[1]

 \item[Server $s$:]
 %\COMMENT{global model $\model$, client models $\{\model_c, \ c\in \clients \}$}
    \FOR{$t\in \{0,...,T-1\}$}
        \STATE{$s$ selects a subset of the clients $\clients^t\subseteq \clients$, }\label{algoline:select_client}
        \STATE{$s$ broadcasts the global model $\model^t$ to %the clients in 
        $\clients^t$,} \label{algoline:broadcast}
        \STATE{$s$ waits for the updated models $\model_c^t$ %returned 
        from every client $c\in \clients^t$,}
        \STATE{$s$ computes $\model^{t+1}$ by aggregating the received updated models.}
        \label{algoline:aggregation}
    \ENDFOR
 \item[Client $c\in \clients$: Input $\model$, Output $\model_c$]
 %\COMMENT{local dataset $\dataset_c$} %, learning rate $\eta$.}
 \WHILE{FL training is not completed}
    \STATE{$c$ listens for the arrival of new global model $\model$,}
   \STATE{$c$ updates its local model:
    $\model_c \leftarrow \localupdaterule^c (\model, \dataset_c)$\label{algoline:updaterule}}
    \STATE{$c$ sends back $\model_c$ to the server.}
 \ENDWHILE
\end{algorithmic}
\end{algorithm}

Let $\globalmodel= \arg\min_{\model \in \real^d} \globallossfunction(\model)$ be a global optimal model, i.e., a minimizer of Problem~\eqref{eq:globalobjective}. 
A general framework to learn such a global model in a federated way is shown in Alg.~\ref{algo:fl}; it generalizes a large number of FL algorithms, including FedAvg~\cite{mcmahan2017communication}, FedProx~\cite{li2018federated}, and FL with different client sampling techniques~\cite{nishio2019client, chen2020optimal, cho2020client}. The model~$\model^T$---the output of Alg.~\ref{algo:fl}---is the tentative solution of Problem~\eqref{eq:globalobjective}. Its performance depends on the specific FL algorithm, which precises how clients are selected in line~\ref{algoline:select_client}, how the updated local models are aggregated in line~\ref{algoline:aggregation}, and how the local update rule works in line~\ref{algoline:updaterule}.
For example, in FedAvg, clients are selected uniformly at random among the available clients, the local models are averaged with constant weights, and the clients perform locally multiple stochastic gradient steps (Alg.~\ref{algo:fedavg} in Appendix~\ref{app:client_update}).
%\fred{Algorithm~\ref{algo:fedavg} is not referenced in the text but used in the proofs. It may be good to reference it either in the text or explicitly at the beginning of the proof App}

% \setlength{\intextsep}{10pt}%

\subsection{Threat Model}\label{subsection:threadmodel}

\subsubsection{Honest-but-curious adversary}
We describe first an honest-but-curious adversary,\footnote{In what follows, we refer to the client using female pronouns and the adversary using male pronouns, respectively.} which is a standard threat model in existing literature~\cite{melis2019exploiting, geiping2020inverting, yin2021see, nasr2019comprehensive}, including the FL one~\cite[Table~7]{openproblems}, 
\cite{attribute_fl_workshop, attribute_fl}. This \emph{passive} adversary, who could be the server itself, is 
knowledgeable about the trained model structure, the loss function, and the training algorithm, and may eavesdrop on communication between the attacked client and the server but does not interfere with the training process. 
%\footnote{
 %   The attribute inference attack (see Sec.~\ref{subsec:attacksbackground}) assumes that the honest-but-curious adversary has also access to public features of samples at client $c$.} 
For instance, during training round $t$, the adversary can inspect the messages exchanged between the server and the attacked client (denoted by $c$), allowing him to recover the parameters of the global model $\model^t$ and the updated client model $\model_c^t(K)$ (Alg.~\ref{algo:fedavg} in Appendix~\ref{app:client_update}). 
Let $\roundsclient \subseteq \{t|c\in\clients^t, \forall t\in {0,\dots,T-1}\}$ denote the set of communication rounds during which the adversary inspects messages exchanged between the server and the attacked client and $\messages_c = \{(\model^t, \model_c^t), \forall t\in \roundsclient\}$ denote the corresponding set of messages.
%It is worth noting that the FL server itself could act as the adversary. %The honest-but-curious adversary is a standard threat model in FL~\cite[Table7]{openproblems} and is commonly considered in existing literature~\cite{melis2019exploiting, geiping2020inverting, wei2020framework, yin2021see, nasr2019comprehensive, attribute_fl, source}. 

When it comes to defenses against such an adversary, it is crucial to understand that traditional measures like encrypted communications are ineffective if the attacker is the FL server.
%Note that encrypted communications are ineffective against the FL server. 
More sophisticated cryptographic techniques like secure aggregation protocols~\cite{bonawitz_secureagg, kadhe2020fastsecagg} allow the server to aggregate local updates without having access to each individual update and, then, do hide the client's updated model $\model_c^t$ from the server. Nevertheless, they come with a significant computation overhead~\cite{quoc2020securetf} and are inefficient for sparse vector aggregation~\cite{openproblems}. Moreover, they are vulnerable to poisoning attacks, as they hinder the server from detecting (and removing) potentially harmful updates from malicious clients~\cite{blanchard2017machine, yin2018byzantine,elmhamdiRobustDistributedLearning2020}. For instance, \citet[Sec.~4.4]{truthSerum} introduce a new class of data poisoning attacks that succeed when training models with secure multiparty computation. Alternatively, Trusted Execution Environments (TEEs) ~\cite{TEE, tee2} provide an encrypted memory region to ensure the code has been executed faithfully and privately. They can then both conceal clients' updated models and defend against poisoning attacks. However, implementing a reliable TEE platform in FL remains an open challenge due to the infrastructure resource constraints and the required communication processes needed to connect verified codes~\cite{openproblems}.


\subsubsection{Malicious adversary} 
%G: I HAVE STREAMLINED THE PRESENTATION. THE OLD TEXT IS BELOW.
We also consider a stronger \emph{active} adversary who can interfere with the training process. Specifically, this adversary can modify the messages sent to the clients and have the clients update models~$\model^t$ concocted to reveal more private information. 
 Let $\mathcal{T}^a_c $ be the set of rounds during which the adversary attacks client $c$ by sending malicious model $\model^t$. 
As above, the adversary could be the server itself. This adversary has been widely considered in the literature on reconstruction attacks~\cite{fishing2022, active_sra} and membership inference attacks~\cite{active_membership, nasr2019comprehensive}. Some studies have also explored the possibility of a malicious adversary modifying the model architecture during training~\cite{robbing, zhao2023loki}, even though such attacks appear to be easily detectable. In this paper, we do not allow the adversary to modify the model architecture. 
%and, therefore, excluded from our consideration.
%G: NOT SURE WHY WE SHOULD MENTION IT, WE ARE CITING THE CORRESPONDING PAPERS. DO WE WANT TO SAY THAT PERHAPS WE COULD CONCEIVE EVEN MORE POWERFUL ATTACKS IN THIS SETTING? BUT OUR FOCUS IS ON RECONSTRUCTING THE LOCAL MODEL, IT IS NOT CLEAR WHAT ADVANTAGES WE WOULD HAVE FROM MODIFYING THE ARCHITECTURE.

% \subsubsection{Malicious adversary} We also consider a stronger adversary case where the adversary is a dishonest central party (server or a third party controlling the server). In addition to all the knowledge acquired in the honest-but-curious case, he interferes with the training process, i.e., he can broadcast arbitrary global model $\model^t$ to clients.  This adversary is widely considered in the existing attacks, including reconstruction attack~\cite{fishing2022, active_sra} and membership inference attack~\cite{active_membership, activepassiveattacks}. 
% Although some studies have explored the possibility of a malicious adversary modifying the model architecture during training~\cite{robbing, zhao2023loki}, such modifications are typically easily detectable and therefore excluded from our consideration. 

For simplicity, we will refer to these two adversaries as passive and active adversaries, respectively, throughout the rest of the paper.

\subsection{Attribute inference attack (AIA) for FL}

AIA leverages public information to deduce private or sensitive attributes~\cite{kasiviswanathan2013power,attribute_fl_workshop, attribute_fl,fredrikson2014privacy,yeom2018privacy}.
For example, an AIA could reconstruct a user's gender from a recommender model by having access to the user's provided ratings.
Formally, each input $\x(i)$ of client $c$ consists of public attributes $\x^p(i)$ and of a sensitive attribute~$s_c(i)$. The target value, assumed to be public, is denoted by $y_c^p(i)$. The adversary, having access to $\{(\x^p(i), y_c^p(i)), i=1,..., S_c\}$ and $\messages_c$, aims to recover the sensitive attributes ${s_c(i)}$.\footnote{In ~\cite{fredrikson2014privacy, yeom2018privacy}, the adversary possesses additional information, including
estimates of the marginals or the joint distribution of the data samples. However, in this paper, we do not consider such a more powerful adversary.}
%~\cite{kasiviswanathan2013power, attribute_fl}.

\subsubsection{Existing gradient-based AIA for FL}\label{subsec:gradient-based} \citet{attribute_fl_workshop} and \citet{attribute_fl} present AIAs specifically designed for the FL context and both passive and active adversaries.
%under both a  honest-but-curious adversary and malicious adversary. 
%G: USE \CITET WHEN IT IS MORE NATURAL TO HAVE THE AUTHORS AS SUBJECT, RATHER THAN "Work \cite{...} presents"
The central idea involves identifying sensitive attribute values that yield virtual gradients closely resembling the client's model updates---referred to as \emph{pseudo-gradients}---in terms of cosine similarity. Formally, the adversary solves the following optimization problem:
{\scriptsize \begin{equation}\label{eq:aia_gradient_based}
  \argmax_{\{s_c(i)\}_{i=1}^{S_c}} \sum_{t\in \mathcal{T}}\textbf{CosSim} \left(\frac{\partial\ell(\model^t, 
    \{(\x^p(i), s_c(i), y_c^p(i))\})}{\partial \model^t}, \model^t-\model_c^t\right), 
\end{equation}}
where $\mathcal{T}\subseteq \mathcal{T}_c$ for 
%an honest-but-curious 
a passive adversary and  $\mathcal{T}\subseteq \mathcal{T}_c \cup \mathcal{T}_c^a$ for an active adversary. 
%malicious adversary. 
The active adversary simply sends back to the targeted client $c$ her own model $\model_c^{(t-1)}$ at each attack round in $\mathcal{T}_c^a$.

\citet{attribute_fl_workshop} and \citet{attribute_fl} assume that the sensitive attributes are categorical and discrete random variables. Nevertheless, problem~\eqref{eq:aia_gradient_based} can be solved efficiently using a gradient method with  %approach using a particular form of 
the reparameterization trick and the Gumbel softmax distribution~\cite{jang2017categorical}. 
%~\cite{DBLP:conf/iclr/MaddisonMT17}. 
From~\eqref{eq:aia_gradient_based}, we observe that, since gradients incorporate information from all samples, the attack performance deteriorates in the presence of a large local dataset.
%This is demonstrated by the experiments in~\cite{attribute_fl}, where 
For example, the attack accuracy almost halves on the Genome dataset for the classification task when the client's local dataset size increases from 50 to 1000 samples~\cite[Table~8]{attribute_fl_workshop}. Our experiment (Figure~\ref{fig:gradient_vs_model}) on a regression task corroborates this finding: when the local dataset size increases from 64 to 256, the attack accuracy drops from $60\%$ to the level of random guessing.
%when  training is through FedAvg with a batch size of 32 and 1 local epoch.
%G: THIS DETAILED INFORMATION COULD GO IN THE CAPTION, BUT NO NEED TO PUT IT HERE, ALSO BECAUSE WE DO NOT PUT THE SAME LEVEL OF DETAILS FOR THE EXPERIMENT IN THE LITERATURE.

%G: I UNDERSTAND THAT WHAT FOLLOWS NEEDS TO BE UPDATED/MODIFIED. I HAVEN'T REVIEWED THEN.
%To our knowledge, no existing work directly addresses the design of AIA under a malicious adversary in FL. However, we can draw insights from recent research on a related reconstruction attack, where the adversary aims to recover the entire training input~\cite{active_sra}. In this scenario, the malicious adversary explicitly alters global model weights so that a neuron in the fully connected layer is activated by only one data sample in the batch. This task is challenging, especially when the adversary does not know the locations of data samples. The authors in~\cite{active_sra} proposed to randomize the global model weights, resulting in more negative weights than positive ones. This approach is effective primarily when the input dimension $d$ is high (e.g., CIFAR10 images with $3072$ pixels) and the batch size is small (e.g., 100 samples), which corresponds to the image classification scenario examined in~\cite{active_sra}. 
%Our analytical result (Theorem~\ref{theo:active_bound}) demonstrates that the success rate of such an attack in FedAvg with full batch $n$ and 1 local epoch,  is $O(\frac{\ln^{d}n}{n})$. This success rate is poor when input dimension $d$ is relatively small compared with $n$ and asymptotically approaches zero as $n$ increases.



\subsubsection{Model-based AIA} As an alternative, the AIA can be executed directly on the model (rather than on the model pseudo-gradients), as initially proposed for  centralized training in~\cite{kasiviswanathan2013power, fredrikson2014privacy}. %Let~$\F_\model$ denote the output of model~$\model$, i.e., a real number for a regression task. 
Given a model $\model$, 
the adversary can infer the sensitive attributes by solving the following optimization problems:
\begin{equation}\label{eq:aia_model_based}
     \argmin_{s_c(i)} \ell(\model,(\x^p(i), s_c(i), y_c^p(i))),\,\,\, \forall i\in\{1,...,S_c\}, 
\end{equation}
%G: THIS FORMULATION SEEMS MORE GENERAL, WHEN APPLIED TO THE LINEAR REGRESSION WE GET THE PREVIOUS EXPRESSION
% \begin{equation}\label{eq:aia_model_based}
%      \argmin_{s_c(i)} ||\F_\model((\x^p(i), s_c(i))) - y_c^p(i) ||_2^2,\,\,\, \forall i\in\{1,...,S_c\}, 
% \end{equation}
%where $y_c^p(i)$ is a real number or a label one-hot-encoding for regression and classification, respectively.

Below we provide theoretical guarantees (Prop.~\ref{prop:attribute_nonprivate}) for the accuracy of the model-based AIAs %(Problem~\eqref{eq:aia_model_based}) 
to least squares regression problems. Our theoretical result 
%supports that model-based AIAs do not suffer from the sensitivity of  gradient-based AIAs to the dataset size, and 
supports that in an FL setting, the adversary may advantageously start by estimating the client's optimal local model, i.e., the model that minimizes the client's empirical loss.

%G: I REMOVED WHAT BELOW AND PUT IN THIS SECTION JUST A SUMMARY BECAUSE WE REPEAT IT IN THE FOLLOWING SECTION AND IT IS BETTER TO WELL DISTINGUISH OUR CONTRIBUTIONS FROM THE STATE OF THE ART.
% In particular, we show that its accuracy approaches 100\% as the model better fits the local data and the importance of the sensitive attribute to the prediction increases.
% %if the model $\model$ fits well the local data or if the sensitive attribute has significant importance on the final prediction, the attack can achieve almost 100\% accuracy. 
% This result suggests that model-based AIA do not suffer the sensitivity of  gradient-based AIA to the dataset size. Furthermore, our theoretical finding motivates the adversary to trigger AIA on a model as close as possible to the optimal local model, i.e., $\localmodel = \arg\min_{\model\in \real^d} \locallossfunction(\model, \localdataset)$, which is more likely to overfit the local dataset.

==> sources/checklist.tex <==
\section*{Reproducibility Checklist}
This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced. Yes
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results. Yes
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper. Yes
\end{itemize}
Does this paper make theoretical contributions? Yes
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. Yes
    \item All novel claims are stated formally. Yes
    \item Proofs of all novel claims are included. Yes
    \item Proof sketches or intuitions are given for complex and/or novel results. Yes
    \item Appropriate citations to theoretical tools used are given. Yes
    \item All theoretical claims are demonstrated empirically to hold. Yes
    \item All experimental code used to eliminate or disprove claims is included. NA
\end{itemize}

Does this paper rely on one or more datasets? Yes
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets. No
    \item All novel datasets introduced in this paper are included in a data appendix. NA
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. NA
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. Yes
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. Yes
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. NA
\end{itemize}


Does this paper include computational experiments? Yes
\begin{itemize}
\item Any code required for pre-processing data is included in the appendix. Yes
\item All source code required for conducting and analyzing the experiments is included in a code appendix. Yes
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. Yes
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. Partial
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. Yes
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. Partial
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. Yes
\item This paper states the number of algorithm runs used to compute each reported result. Yes
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. Yes
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). No
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. Partial
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. Yes
\end{itemize}


==> sources/discussion.tex <==
\section{Discussion and conclusions}
In our work, we have demonstrated the effectiveness of using model-based AIA for federated \emph{regression} tasks, when the attacker can approximate the optimal local model. For an honest-but-curious adversary, we proposed a computationally efficient approach to reconstruct the optimal \emph{linear} local model in least squares regression. In contrast, for neural network scenarios, our passive approach involves directly utilizing the last returned model (Sec.~\ref{subsec:baseline}). We believe more sophisticated reconstruction techniques may exist, and we plan to investigate this aspect in  future work.


%For a linear model with binary cross-entropy loss (\emph{classification task}), it can be shown that the model-based AIA~\eqref{eq:aia_model_based}
 %on a binary sensitive attribute is equivalent to a simple label-based attack, where the attribute is uniquely reconstructed based on the label. This approach leads to poor performance because the attack relies solely on general population characteristics and ignores individual specificities.

The reader may wonder if the superiority of model-based attacks over gradient-based ones also holds for \emph{classification} tasks. Some preliminary experiments we conducted suggest that the relationship is inverted. We advance a partial explanation for this observation.
 For a linear model with binary cross-entropy loss, it can be shown that the model-based AIA  \eqref{eq:aia_model_based} on a binary sensitive attribute is equivalent to a simple label-based attack, where the attribute is uniquely reconstructed based on the label. This approach leads to poor performance because the attack relies only on general population characteristics and ignores individual specificities.
%  More precisely, when $\model[s]>0$, model-based AIA will infer $1$ for the sample with label $1$ and $0$ for the sample with label $0$. 
This observation also holds experimentally for neural networks trained on the Income-L dataset, largely due to the inherent unfairness of the learned models. For example, for the same set of public features, being a man consistently results in a higher probability of being classified as wealthy compared to being a woman. As a consequence, the AIA infers gender solely based on the high or low income label. These preliminary remarks may prompt new interesting perspectives on the relationship between fairness and privacy (see for example the seminal paper~\cite{chang2021privacy}).
 %We want to highlight here that the performance of model-based AIA \eqref{eq:aia_model_based} for \emph{classification} task is closely linked to the fairness of the model. This serves as an example of the observation that ``fairness comes at the cost of privacy"~\cite{chang2021privacy}. 
 
Last but not least, to mitigate privacy leakage, beyond differential privacy mechanisms, there are empirical defenses such as Mixup~\cite{mixup}, which trains a model on composite data samples obtained through linear combinations of sample pairs, and TAPPFL~\cite{aaai_defense}, which learns low-dimensional representations that minimize information about private attributes. However, the effectiveness of these defenses has not yet been demonstrated on \emph{regression} tasks, and we leave this for future work.
 
 

==> sources/introduction.tex <==
\section{Introduction}

Federated learning (FL) enables multiple clients to collaboratively train a global model~\cite{mcmahan2017communication, lian17, li2018federated}. 
Since clients' data is not collected by a third party, FL naturally offers a certain level of privacy. Nevertheless, FL alone does not provide formal privacy guarantees, and recent works have demonstrated that clients' private information can still be easily leaked~\cite{surveyAttacks, liu2022threats}.
For instance, 
%an adversary can infer whether a data sample is used in the training process~\cite{melis2019exploiting,zari2021efficient,active_membership}. 
an adversary with access to the exchanged messages and knowledge of some public information (e.g., client's provided ratings)~\cite{attribute_fl_workshop, attribute_fl, feng2021attribute} can reconstruct a client's sensitive attributes (e.g., gender/religion) in an attack known as attribute inference attack (AIA).
% on the server side can 
%  reconstruct client's sensitive attributes (e.g., gender/religion) by exploiting public information  (e.g., client's provided ratings)~\cite{attribute_fl, feng2021attribute}, known as attribute inference attack (AIA).  
% He can also reconstruct client's training samples such as images~\cite{geiping2020inverting, yin2021see, active_sra}.
%, which is known as attribute inference attack (AIA).
Additionally, the adversary can reconstruct client's training samples such as images~\cite{geiping2020inverting, yin2021see}.
%, which is known as attribute inference attack (AIA).

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.2]{figures/income/dataset_size_effect.png}
    \caption{Average performance of different AIAs
    %two gradient-based AIAs and two model-based AIAs (on the final global model and the optimal local model)
    when four clients train a neural network through FedAvg with 1 local epoch and batch size 32. Each client stores $S_c$ data points randomly sampled from ACS Income dataset~\cite{income_dataset}. The adversary infers the gender attribute of every data sample held by the client given access to the released (public) information.}
    \label{fig:gradient_vs_model}
\end{figure}

However, these reconstruction attacks for FL have primarily been tested on classification tasks and have not been explored for \textit{regression} tasks, which are, needless to say, equally important for practical applications. 
%critical across a wide range of industries for making informed decisions, optimizing processes, and predicting future trends. 
Quite surprisingly, our experiments, as shown in Fig.~\ref{fig:gradient_vs_model}, demonstrate that the accuracy of state-of-the-art gradient-based AIA under a honest-but-curious adversary~\cite{attribute_fl_workshop, attribute_fl} (referred to as passive) drops significantly from $71\%$ on a classification task to $50\%$ (random guess) on a regression task once the targeted client holds more than 256 data points.
Furthermore,  even a more powerful (active) adversary capable of forging the messages to the targeted client to extract more information~\cite{attribute_fl_workshop, attribute_fl} 
%can hardly improve the AIA performance on regression tasks. 
offers only limited improvement to the AIA performance on regression tasks.
Detailed information about this experiment is in Appendix~\ref{app:figure1}. %\todo{add section to appendix}.

% However, these reconstruction attacks for FL have primarily been tested on classification tasks and rarely explored for \textit{regression} tasks, which are critical across a wide range of industries for making informed decisions, optimizing processes, and predicting future trends. Our experiments demonstrate that the accuracy of the latest AIA under a honest-but-curious adversary~\cite{attribute_fl},  drops significantly from $68\%$ on a classification task to $50\%$ (random guess) on a regression task on ACS Adult Income dataset~\cite{income_dataset}.
% \todo{to add some experiment support}
% Furthermore,  even under a stronger adversary capable of tampering with the training process, by isolating the targeted client~\cite{attribute_fl}, the existing AIA can hardly improve the performance  for regression task.

%Furthermore, even under a stronger adversary capable of tampering with the training process, drawing from ideas in existing active attack strategies~\cite{active_sra}, the accuracy of AIA could not be improved, particularly when the local dataset size $n$ exceeds the input dimension $d$. In addition, our analytical analysis (Theorem~\ref{theo:active_bound}) shows that the accuracy of such active attack tends to zero asymptotically w.r.t. $n$, assuming that client's dataset is drawn from a Gaussian distribution as long as $d$ is independent of $n$. 

In this paper, we show that federated training of regression tasks does not inherently enjoy higher privacy, but it is simply more vulnerable to other forms of attacks. While existing FL AIA attacks for classification tasks are gradient-based (see Sec.~\ref{subsec:gradient-based}), we show that model-based AIAs---initially proposed for centralized training~\cite{fredrikson2014privacy, kasiviswanathan2013power, yeom2018privacy}---may be more effective for regression tasks.  Figure~\ref{fig:gradient_vs_model} illustrates that a  model-based attack on the server's global model (i.e., the final model trained through FL) already performs at least as well as the SOTA gradient-based passive attack. Moreover, it highlights that even more powerful attacks (up to 30~p.p.~more accurate) could be launched if the adversary had access to the optimal local model of the targeted client (i.e., a model trained only on the client's dataset).




% Hence, in this paper, we aim to enhance the performance of \textit{AIA} in FL, specifically within the context of \textit{regression tasks}, an area less explored in existing attack literature on FL. Our approach diverges from all existing reconstruction attacks for classification in FL, which primarily rely on gradient-based methods (detailed in Section~\ref{subsec:gradient-based}). Instead, we adopt a model-based AIA approach~\cite{fredrikson2014privacy, kasiviswanathan2013power, yeom2018privacy}, as originally studied in centralized settings.


% Hence, in this paper, we aim to enhance the performance of \textit{AIA} in FL, specifically within the context of \textit{regression tasks}, an area less explored in existing attack literature on FL. Our approach diverges from all existing reconstruction attacks for classification in FL, which primarily rely on gradient-based methods (detailed in Section~\ref{subsec:gradient-based}). Instead, we adopt a model-based AIA approach~\cite{fredrikson2014privacy, kasiviswanathan2013power, yeom2018privacy}, as originally studied in centralized settings.

%However, these model-based attacks are effective only when the model overfits the client's local data, a condition not really met by the global model learned in FL. Due to the heterogeneity of clients' local datasets~\cite{mcmahan2017communication,khaled2020tighter}, 
%the optimal global model and the optimal local one may be far apart~\cite[Figures~2,3]{guo2022fedaug}.  Indeed, our experiment (Figure~\ref{fig:gradient_vs_model}) demonstrates that model-based attack triggered on the global model shows little improvement over existing gradient-based attack~\cite{attribute_fl}. While, if the adversary has access to the optimal local model of targeted client, the model-based AIA can be enhanced by at least $30$~p.p. 
Motivated by these observations, we propose a new two-step model-based AIA for \emph{federated regression tasks}. In this attack, the adversary first (approximately) reconstructs the client's optimal local model and then applies an existing model-based AIA to that model.



% However, these model-based attacks are effective only when the model overfits the client's local data, a condition not met by the models exchanged between FL clients and the server. 
% In fact, in FL, clients cannot perform many local gradient steps between two consecutive communication rounds without the risk of harming convergence of the global model due to the heterogeneity of clients' local datasets~\cite{mcmahan2017communication,khaled2020tighter}. Consequently, the returned models from the clients are far from their local optima. Besides, the optimal global model and the optimal local one may be far apart~\cite[Figures~2,3]{guo2022fedaug}. As such, there is little value in attacks on the global model or the returned models.  Indeed, our experiment (Figure~\ref{fig:gradient_vs_model}) demonstrates that model-based attacks triggered on the global and the last returned model show no significant improvement over existing gradient-based attack~\cite{attribute_fl}. While, if the adversary has access to the optimal local model of targeted client, the model-base AIA can be enhanced by at least $20$ p.p. 







% In this regard, we propose  a new model-based AIA for FL, where the first step is to approximate the optimal local model that a client would have trained using only its local dataset and then apply the classicial model-based AIA approach. 

%we initiate the study of a new attack, called the \textit{local model reconstruction attack} (LMRA), where the adversary seeks to reconstruct the model,. This attack is dangerous as it allows the adversary to trigger the above-mentioned AIA model-based attack with better performance. 
%This attack is potentially very dangerous as its performance doesn’t degrade when the local dataset size increases, allowing the adversary to trigger the above-mentioned model-based attacks with better performance. 
 


%In this paper, we propose a novel model-based attribute inference attack leveraging the local model reconstruction attack, which overcomes the limits of gradient-based attribute inference attacks, i.e, its performance does not decrease as the local dataset size increase. We assume a weak adversary, who is honest-but-curious, i.e, who only eavesdrops the exchanged messages between the client and the server, but does not interfere with the training process.  
%The adversary (e.g., a malicious server) knows the structure of the trained model and the loss function, as well as the training algorithm, as commonly assumed in the literature~\cite{melis2019exploiting, geiping2020inverting, wei2020framework, yin2021see, nasr2019comprehensive}. 

Our main contributions can be summarized as follows:
\begin{itemize}
    \item  We provide an analytical lower bound for model-based AIA accuracy in the least squares regression problem. This result motivates the adversary's strategy to approximate the client's optimal local model in federated regression tasks
    %which motivates the adversary to approximate the client's optimal local model in federated regression task
    (Sec.~\ref{sec:model-based-guarantees}).
    \item   We propose methods for approximating optimal local models where adversaries can either eavesdrop on exchanged messages or directly interfere with the training process (Sec.~\ref{sec:lmra}).  
    \item Our experiments show that our model-based AIAs are better candidates for empirically quantifying privacy leakage for federated regression tasks  (Sec.~\ref{sec:exp}).
\end{itemize}

==> sources/results.tex <==
\section{Experiments}\label{sec:exp}
\subsection{Datasets} \label{subsec:datasets}
\paragraph{Medical~\cite{medical_dataset}.} This dataset includes 1,339 records and 6 features: age, gender, BMI, number of children, smoking status, and region. The \emph{regression} task is to predict each individual's medical charges billed by health insurance. The dataset is  split i.i.d. between 2 clients. 

\paragraph{Income~\cite{income_dataset}.} 
This dataset contains census information from 50 U.S. states and Puerto Rico, spanning from 2014 to 2018. It includes 15 features related to demographic information such as age, occupation, and education level. 
The \emph{regression} task is to predict an individual's income. 
We investigate two FL scenarios, named \mbox{Income-L} and Income-A, respectively. In Income-L, there are 10 clients holding only records from the  state of Louisiana (15,982 records in total). These clients can be viewed as the local entities working for the Louisiana State Census Data Center. We examine various levels of statistical heterogeneity among these local entities, with the splitting strategy detailed in Appendix~\ref{app:datasplit_incomel}. In Income-A, there are 51 clients, each representing a census region and collectively covering all regions. Every client randomly selects 20\% of the data points from the corresponding census region, resulting in a total of 332,900 records.


For all the datasets, each client keeps $90\%$ of its data for training and uses $10\%$ for validation.


%Here, we want to estimate the individual's income given demographic information , given. For the attack, we chose the gender as sensitive feature.
%Due to the large size of 1,664,500 records, we extracted two different subsets of points to use in the experimental evaluation. The first subset contains only datapoints from the Louisiana state, namely 20,406 records, denoted in the experiments as 'Louisiana'. For the second set we considered only the 20\% of points of the original dataset, maintaining the initial data distribution. In the rest of the paper we will refer to this dataset as 'All States'. 



%The second evaluated dataset is the medical cost personal dataset \cite{medical_dataset}, where the goal is to predict the medical charges billed by health insurance. 

\subsection{FL training and attack setup}
In all the experiments, each client follows FedAvg (Alg.~\ref{algo:fedavg} in Appendix~\ref{app:client_update}) to train a \emph{neural network} model with a single hidden layer of 128 neurons, using ReLU as activation function. 
The number of communication rounds is fixed to $T = \lceil 100/E \rceil$ where $E$ is the number of local epochs. Each client participates to all rounds, i.e.,~$\mathcal{T}_c = \{0,...,T-1\}$.
The learning rate is tuned for each training scenario (different datasets and number of local epochs),
%different $E$ and different datasets, 
with values provided in Appendix~\ref{app:hyperparameters}. The passive adversary may eavesdrop all the exchanged messages until the end of the training. 
%, i.e.,~$\mathcal{T}_c = \{1,...,T\}$. 
The active adversary launches the attack after $T$ rounds\footnote{We also examine the impact of the attack's starting round. The results are presented in the Appendix~\ref{app:starting_points}.} for additional $\lceil 10/E \rceil$ and $\lceil 50/E \rceil$ rounds.
%, respectively.
%\todo{Maybe better to have the experiments where the attack is launched earlier.}
Every attack is evaluated over FL trainings from 3 different random seeds.
For Medical dataset, the adversary infers whether a person smokes or not. For Income-L and Income-A datasets, the adversary infers the gender. 
The AIA accuracy is the fraction of the correct inferences over all the samples. 
We have also conducted experiments for federated least squares regression on the same datasets. The results can be found in Appendix~\ref{app:linear_model}. 

\subsection{Baselines and our attack implementation}\label{subsec:baseline}
\paragraph{Gradient-based:}
We compare our method with the (gradient-based) SOTA (Sec.~\ref{subsec:gradient-based}). 
The baseline performance is affected by the set of  inspected rounds~$\mathcal{T}$ considered in~\eqref{eq:aia_gradient_based}. We select the inspected rounds $\mathcal{T}$ based on two criteria: the highest cosine similarity and the best AIA accuracy. In a real attack, the adversary is not expected to know the attack accuracy beforehand.
%for tuning purposes. 
Therefore,  we refer to the attack based on the highest cosine similarity as {\bf{Grad}}  and to the other as {\bf{Grad-w-O}} ({\bf Grad}ient {\bf w}ith {\bf O}racle), as it assumes the existence of an oracle that provides the attack accuracy. The details for the tuning of $\mathcal{T}$ and other hyper-parameter settings can be found in Appendix~~\ref{app:hyperparameters}.
   


\paragraph{Our Attacks:} Our attacks consist of two steps: 1) reconstructing the optimal local model, and 2) executing the model-based AIA~\eqref{eq:aia_model_based}. For the first step, a passive adversary uses the last-returned model from the targeted client, while an active adversary  executes Alg.~\ref{algo:active}. The details of the hyperparameter settings can be found in Appendix~\ref{app:hyperparameters}
.

% \paragraph{Our attack:} Our attack contains two steps: 1) reconstructs the optimal local model, 2) executes the model-based AIA~\eqref{eq:aia_model_based}. For the first step, when the adversary is honest-but-curious, he takes the last-returned model from the targeted client. When the adversary is malicious, he executes Alg.~\ref{algo:active}. The details of its hyperparameters setting can be found in Appendix~\ref{app:hyperparameters}.

\paragraph{Model-based with Oracle (Model-w-O):} 
To provide an upper bound on the performance of our approach, we assume the existence of an oracle that provides the optimal local model for the first step of our attack. In practice, the optimal local model is determined empirically by running Adam for a very large number of iterations.
% We assume the existence of an oracle that provides the optimal local model for the first step of our attack. In our implementation, this optimal local model is evaluated empirically. 
% The results can be considered as an upper bound on the attack accuracy for our approach.
   


\subsection{Experimental results}
%\todoi{I think that even if might be trivial, it should be better to write somewhere how we evaluate the accuracy. (meaning correctly recon / total n samples )}

\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
        \hline
         \multicolumn{2}{|c|}{\bfseries \backslashbox{AIA (\%)}{Datasets}}  & Income-L  &Income-A  &Medical \\
         \hhline{|=|=|=|=|=|}
    \multirow{3}{*}{\bfseries Passive}& Grad&60.36\scriptsize{$\pm$0.67} &54.98\scriptsize{$\pm$0.29} &87.26\scriptsize{$\pm$0.92} \\ 
    & Grad-w-O &71.44\scriptsize{$\pm$0.33}  &\bf{56.10}\scriptsize{$\pm$1.12} &91.06\scriptsize{$\pm$0.55} \\ 
    &Ours &\bf{75.27}\scriptsize{$\pm$0.32}  &55.75\scriptsize{$\pm$0.17}  & \bf{95.90}\scriptsize{$\pm$0.04}\\
    \hhline{|=|=|=|=|=|}
    \multirow{3}{*}{\shortstack[c]{\bfseries Active \\(10 Rnds)}}& Grad&60.24\scriptsize{$\pm$0.60}  &54.98\scriptsize{$\pm$0.29} &87.26\scriptsize{$\pm$0.92} \\ 
       & Grad-w-O &80.69\scriptsize{$\pm$0.55} &56.10\scriptsize{$\pm$1.12} &91.06\scriptsize{$\pm$0.55} \\ 
    & Ours&\bf{82.02}\scriptsize{$\pm$0.85} &\bf{63.53}\scriptsize{$\pm$0.73} &\bf{95.93}\scriptsize{$\pm$0.07} \\
    \hline
    \multirow{3}{*}{\shortstack[c]{\bfseries Active \\(50 Rnds)}}& Grad&60.24\scriptsize{$\pm$0.60}  & 53.36\scriptsize{$\pm$0.40} &87.26\scriptsize{$\pm$0.92} \\ 
     & Grad-w-O &80.69\scriptsize{$\pm$0.55}  &56.12\scriptsize{$\pm$0.12} &91.06\scriptsize{$\pm$0.55} \\ 
    & Ours&\bf{94.31}\scriptsize{$\pm$0.11} &\bf{78.09}\scriptsize{$\pm$0.25} &\bf{96.79}\scriptsize{$\pm$0.79} \\
    \hhline{|=|=|=|=|=|}
    \multicolumn{2}{|c|}{\bfseries Model-w-O}&94.31\scriptsize{$\pm$0.11} &78.31\scriptsize{$\pm$0.07} &96.79\scriptsize{$\pm$0.79} \\ 
    \hline 
    \end{tabular}
    \caption{The AIA accuracy over all clients' local datasets evaluated under both honest-but-curious (passive) and malicious (active) adversaries across  Income-L, Income-A, and Medical FL datasets~(Sec.~\ref{subsec:datasets}). 
    The standard deviation is evaluated over three FL training runs with different random seeds.
    All clients run FedAvg with 1 epoch and batch size 32. For Income-L, we consider the dataset with $40\%$ of data heterogeneity (Appendix~\ref{app:datasplit_incomel}).}
    \label{tab:attacks_32}
\end{table}
%\todo{Needs to be later revised}
 From Table~\ref{tab:attacks_32}, we see that our attacks outperform gradient-based ones in both passive and active scenarios across all three datasets. Notably, our passive attack achieves improvements of over $15$ and $8$ percentage points (p.p.) for the Income-L and Medical datasets, respectively. Even when the gradient-based method has access to an oracle, our passive attack still achieves higher accuracy on two datasets and comes very close on Income-A. When shifting to active attacks, the gains are even more substantial. For instance, when the attack is active for 50 rounds, we achieve gains of 13, 22, and 5 percentage points (p.p.) in Income-L, Income-A, and Medical, respectively, over Grad-w-O, and even larger gains over the more realistic Grad. Furthermore, the attack accuracy reaches the performance expected from an adversary who knows the optimal local model. Interestingly, while our attacks consistently improve as the adversary's capacity increases (moving from a passive attacker to an active one and increasing the number of rounds of the active attack), this is not the case for gradient-based methods. 
 %Specifically, for Grad, additional active rounds do not yield, in most cases, solutions with higher cosine similarity  compared to the passive case. Even when this does occur, as seen once with the Income-A dataset when the adversary attacked for 50 rounds, the resulting attack accuracy may decrease.
 
%  Interestingly, while our attacks consistently improve as the adversary's capacity increases (moving from a passive attacker to an active one and increasing the number of rounds of the active attack), this is not the case for gradient-based methods, whose accuracy marginally increases, if it increases at all, for Grad-w-O and sometimes even decreases for Grad. Indeed, for Grad, additional active rounds do not yield solutions with higher cosine similarity compared to the passive case. Even when this does occur, as seen once with the Income-A dataset when the adversary attacked for 50 rounds, the resulting attack accuracy decreased. We also investigate how the performance of the attacks evolves with an increasing number of active rounds. The results are presented in Appendix~\ref{app:impact_active_rounds}.
 %\todoi{add something for the active Income-A 50 rounds getting worse.}




\begin{figure*}[hbt!]
\begin{minipage}[b]{0.33\linewidth}
\includegraphics[scale=0.2]{figures/income/Heter_effect_louisiana_32.png}
\end{minipage}
\begin{minipage}[b]{0.33\linewidth}
\includegraphics[scale=0.2]{figures/income/batch_size_effect_32.png}
\end{minipage}
\begin{minipage}[b]{0.33\linewidth}
\includegraphics[scale=0.2]{figures/income/local_epochs_effect.png}
\end{minipage}
\caption{The AIA accuracy over all clients' local datasets under different heterogeneity levels (left) ($0\%$ represents i.i.d case), batch sizes (center), and local epochs (right) for Income-L dataset. The default values for heterogeneity level, batch size $B$ and local epochs $E$ are set to $40\%$, $32$, and $1$, respectively. The malicious adversary attacks $\lceil 50/E \rceil$ rounds after $\lceil 100/E \rceil $ communication rounds.
Crosses represent passive attacks, while dots represent active attacks. Dashed lines correspond to gradient-based attacks (Grad), and solid lines correspond to model-based attacks (Ours and Model-w-O).}
    \label{fig:impact}
\end{figure*}




\paragraph{Impact of data heterogeneity.} 
We simulate varying levels of heterogeneity in the Income-L dataset and illustrate how the attack performance evolves in Figure~\ref{fig:impact} (left). First, we observe that as the data is more heterogeneously split, the accuracy of AIA improves for all approaches. 
Indeed, the data splitting strategy (Appendix~\ref{app:datasplit_incomel}) leads to a greater degree of correlation between the clients' sensitive attributes and the target variable at higher levels of heterogeneity. This intrinsic correlation facilitates the operation of all AIAs.
We observe in these experiments, as in previous ones, that active Grad does not necessarily offer advantages over passive Grad. In the more homogeneous case (which is less realistic in an FL setting), our passive attack performs slightly worse than Grad, but its accuracy increases more rapidly with heterogeneity, resulting in an AIA accuracy advantage of over 20 p.p. in the most heterogeneous case.
Our active attack over 50 additional rounds consistently outperforms Grad by at least 30 p.p. and is almost indistinguishable from \mbox{Model-w-O}.


% We observe also in these experiments that active Grad has no advantage w.r.t. passive Grad.
% In the more homogeneous case (which is less realistic in a FL setting), our passive attack performs slightly worse than Grad, but then its accuracy increases faster with heterogeneity,  resulting in an AIA accuracy advantage of over 20 p.p in the extremely heterogeneous case.

% Our passive attack benefits from a In the passive scenario, our approach exhibits a faster growth in comparison to Grad, resulting in an AIA accuracy advantage of over 20 p.p in the extreme heterogeneous case. In the more homogeneous case (which is less realistic in a FL setting), our approach performs slightly worse than Grad. For active attacks with 50 additional rounds, our attack consistently outperforms Grad by at least 30 p.p. and approaches Model-w-O, the performance under an adversary who knows the optimal local model.


\paragraph{Impact of batch size.} 
%We test the FedAvg training with 1 local epoch and 6 different batch sizes. 
Figure~\ref{fig:impact} (center) shows that the performance of our attacks slightly decrease as the batch size increases.  A possible explanation for this is that a larger batch size results in fewer local updates per epoch, leading the client to return a less overfitted model. Despite this, our approach consistently outperforms Grad in all cases.
%This is due to the fact that a larger batch size results in fewer local updates per epoch, leading to the client returning a less over-fitting model. Despite this, our approach consistently outperforms Grad in all cases.

\paragraph{Impact of the number of local epochs.}
%We test the FedAvg training with batch size 32 and 5 different local epochs. 
Figure~\ref{fig:impact} (right) shows that under passive attacks, our approach is not sensitive to the number of local epochs, whereas Grad's performance deteriorates to the level of random guessing as the number of local epochs increases to 5. Interestingly, active Grad significantly improves upon passive Grad as the number of local epochs increases. While our active approach progressively performs slightly worse, it still maintains an advantage of over 10 p.p.~compared to Grad.


%, we observe that under passive attacks, our approach remains stable, while Grad's performance deteriorates to a random guess as the number of local epochs increases to 5. For active attacks, our approach performs slightly worse as the number of local epoch increases, but still maintains an advantage of over 10 percentage points compared to Grad.

% \paragraph{Impact of the local dataset size.}\mbox{}\\
% \begin{minipage}{0.32\linewidth}
% The figure on the right shows 
% how each client's dataset size impacts individual (active) AIA accuracy in Income-A dataset. The experiment setting is the same as in Table~\ref{tab:attacks_32} with  50 active rounds. 

% \end{minipage}
% \begin{minipage}{0.65\linewidth}
%     \centering
%     \includegraphics[scale=0.18]{figures/income/client_acc_scatterplot.png}
%     %\captionof{figure}{The active AIA accuracy on each client's dataset vs client's local dataset size  in Income-A dataset.  The batch size and the active rounds are set to $32$ and $50$, respectively.  }
%     \label{fig:dataset_size_effect}
% \end{minipage}

\paragraph{Impact of the local dataset size.}
Figure~\ref{fig:dataset_size_effect} shows how each client's dataset size impacts individual (active) AIA accuracy in Income-A dataset. %The experiment setting is the same as in Table~\ref{tab:attacks_32} with  50 active rounds.
We observe that for all methods, clients with smaller datasets are more vulnerable to the attacks,  
%Because the corresponding gradients incorporate less samples and 
because the models overfit the dataset more easily. 
Moreover, for clients with more than 20000 data points, Grad provides an attack performance close to random guessing.
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.18]{figures/income/client_acc_scatterplot.png}
    \caption{AIA accuracy in Income-A dataset on clients with different local dataset size $S_c$. The experiment setting is the same as in Table~\ref{tab:attacks_32} with  50 active rounds.}
    \label{fig:dataset_size_effect}
\end{figure}
% Figure~\ref{fig:dataset_size_effect} shows how each client's dataset size impacts individual (active) AIA accuracy in Income-A dataset. The experiment setting is the same as in Table~\ref{tab:attacks_32} with  50 active rounds.
% We observe that for all methods, clients with smaller datasets are more vulnerable to the attacks,  
% %Because the corresponding gradients incorporate less samples and 
% because the models overfit the dataset more easily. 
% Moreover, for clients with more than 20000 data points, Grad provides an attack performance close to random guessing.


\paragraph{Impact of defense mechanisms.}
To mitigate privacy leakage, we %extend the 
apply a federated version of DP-SGD~\cite{DP}, which provides sample-level differential privacy guarantees~\cite{Dwork, slDP}. 
%This method provides theoretical guarantees on the privacy budget ($\epsilon, \delta$) in terms of sample-level differential privacy.
Our experiments show that even with this defense mechanism in place, our approach still outperforms the baselines in most of the scenarios.  The  results are in Appendix~\ref{app:defense}.



% \begin{table}[t]
% % \renewcommand{\arraystretch}{1.3}
%     \caption{FedAdam}
%     \label{table: FedAdam}
%     \centering
%     \begin{tabular}{c||c||c||c||c}
%     \hline
%     \bfseries Dataset & \bfseries Gradient Based & \bfseries Global Model & \bfseries Last Returned Model & \bfseries Active \\ 
%     \hline\hline
%     Income (Louisiana) & 59.90\% & 62.37\% & 69.41\% & 85.67\% \\
%     \hline
%     Income (All states) & 53.73\% & 57.06\% & 58.4\% & 83.84\% \\
%     \hline
%     Income (Large) & 52.35\% & 60.94\% & 62.24\% & 71.53\% \\
%     \hline
%     Medical Cost  & 87.79\% & 96.34\% & 96.42\% & 96.68\% \\
%     \hline
%     \hline
%     \end{tabular}
% \end{table}

% \begin{table}[t]
% % \renewcommand{\arraystretch}{1.3}
%     \caption{Linear FedAvg}
%     \label{table: FedAvg}
%     \centering
%     \begin{tabular}{c||c|c|c|c}
%     \hline
%     \bfseries Dataset & \bfseries Gradient & \bfseries Global  & \bfseries Last Returned & \bfseries Active \\ 
%     \hline\hline
%     Income (Louisiana) &  \\
%     \hline
%     Income (All states) &  \\
%     \hline
%     Income (Large) \\
%     \hline
%     Medical Cost   \\
%      \hline
%      \hline
%      \end{tabular}
%  \end{table}


% \begin{table*}[t]
% % \renewcommand{\arraystretch}{1.3}
%     \caption{FedAvg: B=32}
%     \label{table: FedAvg 32}
%     \centering
%     \begin{tabular}{c||c|c|c|c|c|c|}
%     \hline
%     Thread Model& \multicolumn{3}{c|}{Passive} &  \multicolumn{3}{c|}{Active} \\
%     \hline
%     \bfseries Dataset & \bfseries Passive Gradient & \bfseries Global  & \bfseries Last Returned & \bfseries Gradient/Ours (5)& \bfseries Gradient/Ours (10) & \bfseries Gradient/Ours (50) \\ 
%     \hline
%     Income (Louisiana) & 63.96\% & 58.69\% & 65.93\% & 87.26\% & & \\
%     \hline
%     Income (All states) & 56.12\% & 56.91\% & 56.47\% & 82.49\% & & \\
%     \hline
%     Income (Large) & 54.80\% & 55.63\% & 56.05\% & 70.77\% 
%     & & \\\hline
%     Medical Cost & 52.74\%  & 96.01\% & 96.18\% & 96.68 \% & &\\
%      \hline
%      \hline
%      \end{tabular}
%  \end{table*}

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.3]{figures/income/batch_size_effect_32.png}
%     \caption{The average performance of attribute inference attacks with different batch sizes $B$ on the Louisiana dataset with heterogeneity 40\%. Lines marked with dots indicate an active attacker, while the crosses indicate a passive attacker. The green line with triangles shows the performance of the empirical optimal model. Active results are reported after 50 additional communication rounds.}
%     \label{fig:enter-label}
% \end{figure}


